A Hybrid Neural Network Model for Commonsense Reasoning

This paper proposes a hybrid neural network (HNN) model for commonsense reasoning. An HNN consists of two component models, a masked language model and a semantic similarity model, which share a BERT-based contextual encoder but use different model-specific input and output layers. HNN obtains new state-of-the-art results on three classic commonsense reasoning tasks, pushing the WNLI benchmark to 89%, the Winograd Schema Challenge (WSC) benchmark to 75.1%, and the PDP60 benchmark to 90.0%. An ablation study shows that language models and semantic similarity models are complementary approaches to commonsense reasoning, and HNN effectively combines the strengths of both. The code and pre-trained models will be publicly available at https://github.com/namisan/mt-dnn.

==> background.tex <==
\section{Background}
\label{background}

\subsection{Pronoun resolving tasks}
Winograd Schema Challenge is a well-known tasks that target to resolve the pronoun in the sentence to the correct antecendent given several candidates. Those tasks are easy for humans but hard for machines. The latest number of this task is 72 which is based on language model trick. Due to the hardness of this task, it's thought of one of the Turning-Alternative tasks. WNLI is a new task derived from WSC but formulated as a NLI task instead of ranking task. It's the hardest task in all the 9 tasks in GLUE. 


\textbf{TODO: Add examples}

\begin{table}[htb]
\renewcommand\thetable{1} 
\begin{tabular}{p{0.01\textwidth} p{0.35\textwidth} p{0.15\textwidth}}
1. & \textit{The city councilmen refused the demonstrators a permit because \textbf{they} \textbf{feared} violence.} & \textit{\textbf{The city councilmen}} \\\\
 & \textit{The city councilmen refused the demonstrators a permit because \textbf{they} \textbf{advocated} violence.}  & \textit{\textbf{the demonstrators}} \\\hline
2. & \textit{Joe has sold his house and bought a new one a few miles away. He will be \textbf{moving into} \textbf{it} on Thursday.} & \textit{\textbf{the new house}} \\\\  
 & \textit{Joe has sold his house and bought a new one a few miles away. He will be \textbf{moving out of} \textbf{it} on Thursday.} & \textit{\textbf{the old house}} \\\hline   
\end{tabular}
 \caption{Examples}
 \label{example}
\end{table}


\subsection{BERT}
BERT is a transformer based bidirectional language model with good performance on many down streaming tasks. It only use attention unit in the whole structure instead of using LSTM or CNN. 


\textbf{TODO: Add introductin to BERT, espcially the attention unit}

\subsection{Attention}
With attention, it will be easier for us to understand how the network works. In BERT, each token's output at current layer is a weighted sum of previous tokens while the weight is calculated via attention. Wihtout fine-tuning, the weight are almost equally distributed among the tokens in the sentence.

\textbf{TODO: add example to show the observation}. 

So it's hard to distinguish the pronoun between antecedent and other candidates. But if we can make the attention of the pronoun more concentrated on the true antecedent, then it will be easy for us to find out the correct candidate just by comparing the representations. Because in this case, the weight will be dominated by the antecedent which will result a high similarity between the representations.


\textbf{TODO: add example and formula to demonstrate }


\textbf{TODO: start with single token pronoun, extend to multi-token pronoun -\textgreater attentive pooling}

With this motivation, we proposed a new method to resolve the pronoun in a more explainable way instead of previous language model trick.


==> problem.tex <==
\section{Problem}

\JG{I suggest we remove this section, but infuse the content into section 3 and/or the experiment section.}

WSC273 and PDP60 tasks can be category into pronoun coreference resolving task. Given a sentence $\mathbf{S}$ which contains at least one pronoun, a pronoun $\mathbf{P}$ from $\mathbf{S}$ and several possible antecedent candidates $\left\{\mathbf{A_i}\right\}_{\times n}$, the task is to find out which candidate is the antecedent of the pronoun. There are $2$ candidates for each pronoun in WSC273 and $2\thicksim5$ candidates in PDP60. 

WNLI task is derived from WSC273, but it formulates the task into a NLI task. For each premise sentence, a sub-sentence is created by replace the pronoun in the original sentence with a possible antecedent as shown in table \ref{example}. The sub-sentence is called hypothesis. The task is to determine if these two sentences are entailed or not. 

\cite{kocijan2019surprisingly} reformulate WNLI task back into task similar to WSC273 by extracting all nouns from the premise as the candidates, and use the same way to solve this task. However, this method has some limitations. First, the noun extraction is not accurate as the antecedent might be a noun phrase instead of a noun and the extraction accuracy is determined by external tool. Second, in some cases, the antecedent in the hypothesis is not a direct copy of the noun phrase in the premise. That means there might be semantically duplicated candidates in the list. \todo{Show examples} 

We formulate WNLI as binary classification task which is more close to the original setting and don't need to extract nouns from the premise as candidates. More details will be described in section \ref{sec:ssm}. 

==> related.tex <==
\section{Acknowledgements}
\label{sec:akn}

We would like to thanks Jade Huang from Microsoft for her generous help on this work.

==> training.tex <==
\section{Training}
\label{sec:train}



